Towards Reliable Neural Specifications

Having reliable specifications is an unavoidable challenge in achieving verifiable correctness, robustness, and interpretability of AI systems. Existing specifications for neural networks are in the paradigm of data as specification. That is, the local neighborhood centering around a reference input is considered to be correct (or robust). While existing specifications contribute to verifying adversarial robustness, a significant problem in many research domains, our empirical study shows that those verified regions are somewhat tight, and thus fail to allow verification of test set inputs, making them impractical for some real-world applications. To this end, we propose a new family of specifications called neural representation as specification, which uses the intrinsic information of neural networks - neural activation patterns (NAPs), rather than input data to specify the correctness and/or robustness of neural network predictions. We present a simple statistical approach to mining neural activation patterns. To show the effectiveness of discovered NAPs, we formally verify several important properties, such as various types of misclassifications will never happen for a given NAP, and there is no ambiguity between different NAPs. We show that by using NAP, we can verify a significant region of the input space, while still recalling 84% of the data on MNIST. Moreover, we can push the verifiable bound to 10 times larger on the CIFAR10 benchmark. Thus, we argue that NAPs can potentially be used as a more reliable and extensible specification for neural network verification.

==> Extras.tex <==


\citet{NAPs1} proposes a method to extract and visualize neural activation patterns from pre-trained models.

Those methods share the same idea: prioritizing visualization for explanation. This idea limits what can be evaluated and compared between different methods, since usually a human study is required. Our method tackle the 

They show how different model reacts to different inputs and see how the information on images is processed across the layers. Also, with concepts discovered by analyzing the NAPs of layers, they allow the comparison between models with different architectures for the building-up of classifications across layers. Another similar utilization is, by considering the activation difference between layers as a component to measure if and how the features are evident for or against predictions, providing users with a view of the focus of each layer on images to make decisions with the visualization of activation patterns \citep{zintgraf2017visualizing}. This idea can also apply to domains other than images. Prototypes of Temporally Activated Patterns (PTAP) is a method leveraging activation patterns and their visualization to identify the shapes focused during decision making which helps understand how deep neural networks lean time series data intelligibly \citep{cho2021interpreting}.


In the attempt to explain deep neural network models, few work have focused the attention to the interpretation of the behavior of neural activation patterns \cite{}. 


\textbf{Neural Network Activation Patterns}Neural network activation patterns(NAPs) can help decipher the inner working of neural networks and help individual of interest understand what is learnt by the model. NAPs visualize learned layer concepts. 
    
Current work on NAPs extract similar activation profiles with high-dimensional activation space of a neural network layer and find groups of inputs that are treated similarly. Existing tools can extract NAPs from pre-trained models and provide a visual introspection tool to help analyze NAPs. \cite{NAPs1} 

Neural networks have been playing a significant role in solving various problems. However, the essence of how networks make decisions is still quite unclear to the public, which causes some potential obstacles to adopting neural networks in certain areas such as healthcare and automated drive system. To decipher what has been learned by the inner layer of the neural network, \citet{NAPs1} proposed a methodology and a visual introspection tool to extract neural activation patterns(NAPs) from pre-trained models and analyze them. With the visual analysis of NAPs, we are able to inspect and explain how a model reacts to different inputs and see how the information on images is processed across the layers. Also, with concepts discovered by analyzing the NAPs of layers, they allow the comparison between models with different architectures for the building-up of classifications across layers. Another similar utilization is, by considering the activation difference between layers as a component to measure if and how the features are evident for or against predictions, providing users with a view of the focus of each layer on images to make decisions with the visualization of activation patterns \citep{zintgraf2017visualizing}. This idea can also apply to domains other than images. Prototypes of Temporally Activated Patterns (PTAP) is a method leveraging activation patterns and their visualization to identify the shapes focused during decision making which helps understand how deep neural networks lean time series data intelligibly \citep{cho2021interpreting}.  Apart from analyzing the inner behaviour of a model, activation patterns can also be used for examining the reliability of a decision by checking the similarity of the activation pattern generated during the prediction process with existing patterns extracted from training data, and it can alert to potential misclassification when the similarity is low \citep{cheng2019runtime}.

Verify with NAP. 


==> FigMisclassify1.tex <==
% \begin{figure}[th]
%      \centering
%      \begin{subfigure}[t]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred1_gt6_idx438.pdf}
%          \caption{A testing image from MNIST with ground truth 6, classified as 1}
%          \label{fig:misclsfy_6_to_1}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred1_gt7_idx129.pdf}
%          \caption{A testing image from MNIST with ground truth 7, classified as 1}
%          \label{fig:misclsfy_7_to_1}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred1_gt9_idx229.pdf}
%          \caption{A testing image from MNIST with ground truth 9, classified as 1}
%          \label{fig:misclsfy_9_to_1}
%      \end{subfigure}
%         \caption{Some interesting test images from MNIST that are misclassified as 1 and also follow the $\NAP$ of class 1.}
%         \label{fig:Misclassify_to_1}
% \end{figure}

==> marabou_mnist.tex <==


\begin{table}[t]
\caption{The maximum overlap ratio of dominant pattern for each label (class) on a given $\delta$ for MNIST. Each cell is obtained by $\max_i |N_{col}^{\delta} \bigcap N_i^{\delta}|/ |N_{col}^{\delta}|$ where $N_{col}^{\delta}$ is the set of neurons in the dominant pattern for the label (class) in the header of the column of the selected cell with the given $\delta$, $N_i$ is the set of neurons in the dominant pattern for the label (class) $i$ with the given $\delta$.} 
\label{tab:mnist_max_overlap_ratio}
\begin{center}
\begin{tabular}{ |c || c c c c c c c c c c| }
 \hline
& label0& label1& label2& label3& label4& label5& label6& label7& label8&label9\\
\hline\hline
0.000&0.959 &0.928 &0.963 &0.966 &0.972 &0.973 &0.930 &0.965 &0.957 &0.981\\ 
 \hline
0.010&0.844 &0.834 &0.911 &0.901 &0.881 &0.898 &0.895 &0.884 &0.880 &0.908\\ 
 \hline
0.050&0.864 &0.885 &0.909 &0.904 &0.915 &0.908 &0.899 &0.897 &0.890 &0.893\\ 
 \hline
0.100&0.877 &0.900 &0.910 &0.901 &0.921 &0.910 &0.890 &0.899 &0.900 &0.901\\ 
 \hline
0.150&0.876 &0.904 &0.904 &0.900 &0.919 &0.913 &0.893 &0.907 &0.904 &0.900\\ 
 \hline
0.250&0.893 &0.922 &0.913 &0.912 &0.928 &0.925 &0.905 &0.916 &0.916 &0.913\\ 
 \hline
0.500&0.903 &0.905 &0.925 &0.923 &0.926 &0.923 &0.907 &0.918 &0.927 &0.927\\ 
 \hline
\end{tabular}
\end{center}
\end{table}


==> nap_augmented_prop.tex <==
\begin{table}[t]
\caption{MOVE TO APPENDIX! Searching for adversarial examples for each label within the $L_\infty$ norm-balls of radius 0.1 ($\epsilon = 0.1$) centered at 0. Each column represents a label to be checked. The first row doesn't take NAPs into consideration, the remaining rows use NAPs of different $\delta$s. We report Y if no adversarial examples are found, N otherwise. }

\allen[Be careful with the meaning of Y and N.]
\label{tab:effect_of_delta}
\begin{center}
\begin{tabular}{ |l || r r r r r r r r r r| }
 \hline
& 0& 1& 2& 3& 4& 5& 6& 7& 8& 9\\
\hline\hline
$\epsilon = 0.1$&N &N &N &N &N &N &N &N &N &N \\  
 \hline
$\epsilon = 0.1, \delta = 0.00$&N &N &N &N &N &N &N &N &N &N \\  
 \hline
$\epsilon = 0.1, \delta = 0.01$&N &N &N &N &N &N &N &N &N &N \\ 
\hline
$\epsilon = 0.1, \delta = 0.05$&N &N &N &N &N &N &N &N &N &N \\ 
\hline
$\epsilon = 0.1, \delta = 0.10$&N &N &N &N &N &N &N &N &N &N \\ 
\hline
$\epsilon = 0.1, \delta = 0.15$&N &N &N &N &N &N &N &N &N &N \\ 
\hline
$\epsilon = 0.1, \delta = 0.25$&N &N &N &N &N &N &N &N &N &N \\ 
\hline
$\epsilon = 0.1, \delta =0.50$&\Y &\Y &\Y &N &\Y &\Y &\Y &\Y &\Y &\Y \\ 
\hline

\end{tabular}
\end{center}
\end{table}


==> table_cifar10.tex <==
% at delta =0.05
% 1783	0.012	 unsat
% 6413	0.012	 sat
% 1189	0.012	 unsat
% 8498	0.012	 sat
% 7076	0.012	 unsat
% 1783	0.024	 TIMEOUT
% 6413	0.024	 sat
% 1189	0.024	 unsat
% 8498	0.024	 sat
% 7076	0.024	 sat
% 596	0.024	 TIMEOUT
% 9228	0.024	 unsat

% at delta =0.1
% 1783	0.012	 unsat
% 6413	0.012	 unsat
% 1189	0.012	 unsat
% 8498	0.012	 sat
% 7076	0.012	 unsat
% 1783	0.024	 unsat
% 6413	0.024	 unsat
% 1189	0.024	 unsat
% 8498	0.024	 sat
% 7076	0.024	 sat
% 596	0.024	 unsat
% 9228	0.024	 unsat

\begin{table}
\caption{Augmented robustness with CIFAR10 and CNN.}
\label{tab:cifar10_augmented_NAP}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{$\epsilon$} & \multicolumn{3}{c|}{0.012} & \multicolumn{3}{c|}{0.024} & \multicolumn{3}{c|}{0.12}\\
\cline{2-10}
\multicolumn{1}{|c|}{$\delta$} & 0.99 & 0.95 & 0.9 & 0.99 & 0.95 & 0.9 & 0.99 & 0.95 & 0.9\\
\hline
$\cC(x_0)=8$   &\Y &\Y &\Y &N  &T/o  &\Y &T/o &\Y &\Y\\
$\cC(x_1)=6$   &T/o &N &\Y &N  &N  &\Y &N &N &\Y\\
$\cC(x_2)=0$   &\Y &\Y &\Y &\Y  &\Y  &\Y &N &N &N\\
$\cC(x_3)=1$   &N &N &N &N  &N  &N &N &N &N\\
$\cC(x_4)=9$   &N &\Y &\Y &N  &N  &N &N &N &N\\
$\cC(x_5)=7$   &\Y &\Y &\Y &N  &T/o  &\Y &N &\Y &\Y\\
$\cC(x_6)=3$   &\Y &\Y &\Y &\Y  &\Y  &\Y &N &N &N\\
\hline
\end{tabular}
}
\end{center}
\end{table}
